Towards the glueball spectrum from unquenched lattice QCD

We use a variational technique to study heavy glueballs on gauge configurations generated with 2+1 flavours of ASQTAD improved staggered fermions. The variational technique includes glueball scattering states. The measurements were made using 2150 configurations at 0.092 fm with a pion mass of 360 MeV. We report masses for 10 glueball states. We discuss the prospects for unquenched lattice QCD calculations of the oddballs.

==> tab_fine_spectrum.tex <==
\begin{table}[ht]
  \centering
  \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    Ch. & $t_{\rm min}-t_{\rm max}$ & $am$ & $|c_0|^2$ & $\chi^2/{\rm dof}$ & ${\rm mix}_G$ & ${\rm mix}_S$ & ${\rm mix}_T$ \\
    \hline    \hline
    $A_1^{++}$ & 1-5 & 0.839(28) & 0.94(3) & 0.23 & 0.6874 & 0.2661 & 0.0466 \\
    $A_1^{++\star}$ & 1-5 & 1.447(55) & 0.98(5) & 0.48 & 0.6779 & 0.2611 & 0.0609 \\
    $A_1^{++\star\star}$ & 1-4 & 1.75(11) & 0.88(10) & 0.91 & 0.6865 & 0.2124 & 0.1010 \\
    $A_1^{++\star\star\star}$ & 1-5 & 1.99(12) & 1.16(14) & 0.91 & 0.6727 & 0.2055 & 0.1217 \\
    \hline
    $A_1^{+-}$ & 1-5 & 2.55(39) & 0.99(38) & 0.31 & 0.7207 & 0.2461 & 0.0331 \\
    \hline
    $A_1^{-+}$ & 1-6 & 1.30(4) & 0.89(3) & 0.15 & 0.3257 & 0.0908 & 0.5835 \\
 $A_1^{-+\star}$ & 1-5 & 1.57(8) & 0.73(6) & 0.79 & 0.4919 & 0.1284 &
    0.3797 \\
 $A_1^{-+\star\star}$ & 1-5 & 2.10(28) & 0.76(20) & 0.97 & 0.6800 & 0.1605 & 0.1595 \\
    \hline
    $A_1^{--}$ & 1-4 & 2.41(47) & 0.81(39) & 0.64 & 0.7263 & 0.2486 & 0.0251 \\
    \hline
    $A_2^{++}$ & 1-4 & 1.94(13) & 0.99(13) & 0.30 & 0.7509 & 0.1995 & 0.0495 \\
    \hline
    $A_2^{++}$ & 1-4 & 2.36(30) & 1.08(33) & 0.06 & 0.7086  & 0.1708 & 0.1206 \\
    \hline
    $A_2^{+-}$ & 1-5 & 1.70(10) & 0.76(8) & 0.48 & 0.8366 & 0.0284 &
    0.1350 \\
    $A_2^{+-\star}$ & 1-3 & 2.06(10) & 0.79(15) & 0.41 & 0.8850 & 0.0535 & 0.061 \\
    \hline
    $A_2^{-+}$ & 1-4 & 2.03(20) & 0.66(13) & 0.56
 & 0.8528  & 0.1067 & 0.0405 \\
    $A_2^{-+\star}$ & 1-4 & 2.74(56) & 0.97(60) & 1.03 & 0.8528 & 0.1067 & 0.0405 \\
    \hline
    $A_2^{--}$ & 1-5 & 2.32(25) & 0.98(25) & 1.10 & 0.5526 & 0.3905 & 0.0569 \\
    \hline
    $E^{++}$ & 1-5 & 1.202(32) & 0.86(3) & 0.97 & 0.8117 & 0.1622 & 0.0261 \\
    % 2-5 1.0436 0.0996 0.607 0.124 0.05 0.48 0.8117 0.1622 0.0261
    % 1-3 1.1695 0.0412 0.885 0.034 3.30 1.94 0.8651 0.0718 0.0631
    % 2-5 0.9069 0.0829 0.500 0.082 0.60 1.55 0.8651 0.0718 0.0631
    $E^{++\star}$ & 1-5 & 1.606(87) & 0.89(8) & 0.44 & 0.8457 & 0.1213 & 0.0330 \\
    % 2-5 1.3253 0.3975 0.501 0.392 0.86 1.91 0.8457 0.1213 0.0330
    %1-5 1.6208 0.0959 0.857 0.078 1.57 2.15 0.7316 0.1939 0.0745
    \hline
    $E^{+-}$ & 1-4 & 2.42(40) & 0.98(39) & 0.01 & 0.4243 & 0.1398 & 0.4359 \\
    \hline
    $E^{-+}$ & 1-5 & 1.42(6) & 0.76(5) & 0.76 & 0.4243  & 0.1398 &
    0.4359 \\
    $E^{-+\star}$ & 1-3 & 1.71(10) & 0.81(8) & 0.57 & 0.6943 & 0.0143 & 0.2914 \\
    \hline
 $E^{--}$ & 1-5 & 1.86(19) & 0.71(13) & 1.1 & 0.7984 & 0.1586 & 0.0430 \\
$E^{--\star}$ & 1-5 & 2.08(22) & 0.83(18) & 0.92 & 0.8411 & 0.1464 & 0.0126 \\
    \hline
    $T_1^{++}$ & 1-4 & 2.03(16) & 0.92(15) & 0.90 & 0.9011 & 0.0327 & 0.0662 \\
    \hline
$T_1^{+-}$ & 1-5 & 1.530(71) & 0.86(6) & 0.45 & 0.8870 & 0.0689 & 0.0441 \\
%%$T_1^{+-\star}$ & 1-5 & 1.53(7) & 0.83(5) & 0.46 & 0.8559 & 0.0545 & 0.0897 \\
$T_1^{+-\star}$ & 1-4 & 1.65(7) & 0.87(6) & 0.26 & 0.9277 & 0.0371 & 0.0352 \\
    % 1-4 1.7174 0.1055 0.726 0.076 0.94 1.82 0.8844 0.0483 0.0673
    \hline
    $T_1^{-+}$ & 1-5 & 2.16(26) & 0.89(23) & 0.24 & 0.6700 & 0.2759 & 0.0541 \\
$T_1^{-+\star}$ & 1-5 & 2.21(28) & 0.85(24) & 1.15 & 0.8308 & 0.1114 & 0.0578 \\
    \hline
    $T_1^{--}$ & 1-5 & 2.25(32) & 0.96(31) & 0.33 & 0.7504 & 0.1645 & 0.0851 \\
    \hline
$T_2^{++}$ & 1-4 & 1.238(43) & 0.92(4) & 0.63 & 0.9640 & 0.0144 & 0.0216 \\
$T_2^{++\star}$ & 1-4 & 1.723(70) & 0.92(6) & 0.85 & 0.9551 & 0.0291 & 0.0159 \\
    \hline
%%$T_2^{+-}$ & 1-5 & 1.94(14) & 0.91(13) & 0.57 & 0.8848 & 0.0856 & 0.0296 \\
$T_2^{+-}$ & 1-4 & 1.90(16) & 0.83(13) & 0.99 & 0.8336 & 0.0504 & 0.1160 \\
$T_2^{+-\star}$ & 1-4 & 2.28(29) & 0.94(26) & 0.92 & 0.9249 & 0.0350 & 0.0401 \\
    \hline
$T_2^{-+}$ & 1-4 & 1.50(8) & 0.76(6) & 0.93 & 0.8101 & 0.1736 & 0.0163 \\
$T_2^{-+\star}$ & 1-5 & 1.69(12) & 0.90(10) & 0.28 & 0.3989 & 0.5795 &
    0.0217 \\
    \hline
$T_2^{--}$ & 1-4 & 2.35(26) & 1.07(26) & 0.91 & 0.5124 & 0.3946 & 0.0930 \\
    \hline
    \hline
  \end{tabular}
  \caption{Spectrum on the ensemble of Tab.~\ref{tb:ensemble}. For
    each state we were able to extract a signal, we show the
    parameters of the fit with Eq.~\eqref{eq:coshFIT} and the relative
    projection of the mass eigenstate on the different subsets of
    operators (${\rm mix}_G$, ${\rm mix}_S$, ${\rm mix}_T$). Good
    overlaps $|c_0|^2 \sim {\cal O}(1)$ and $\chi^2/{\rm dof}$ are
    shown.}
  \label{tab:spectrum-fine}
\end{table}

